Cost-Aware Robust Tree Ensembles for Security Applications

There are various costs for attackers to manipulate the features of security classifiers. The costs are asymmetric across features and to the directions of changes, which cannot be precisely captured by existing cost models based on $L_p$-norm robustness. In this paper, we utilize such domain knowledge to increase the attack cost of evading classifiers, specifically, tree ensemble models that are widely used by security tasks. We propose a new cost modeling method to capture the feature manipulation cost as constraint, and then we integrate the cost-driven constraint into the node construction process to train robust tree ensembles. During the training process, we use the constraint to find data points that are likely to be perturbed given the feature manipulation cost, and we use a new robust training algorithm to optimize the quality of the trees. Our cost-aware training method can be applied to different types of tree ensembles, including gradient boosted decision trees and random forest models. Using Twitter spam detection as the case study, our evaluation results show that we can increase the attack cost by 10.6X compared to the baseline. Moreover, our robust training method using cost-driven constraint can achieve higher accuracy, lower false positive rate, and stronger cost-aware robustness than the state-of-the-art training method using $L_\infty$-norm cost model. Our code is available at https://github.com/surrealyz/growtrees.

==> discussion.tex <==
\section{Discussion}

\subsection{False positive rate} It is a known tradeoff that increasing the robustness
of a classifier may decrease its regular test accuracy and increase the false positive rate.
As shown in evaluation and the twitter spam case study, the more robust a model is,
the higher the false positive rate. In security applications, it is especially important
to maintain low false positive rate so as to not trigger too many false alarms for threat
analysts every day. How to improve the false positive rate of the robust models
will be a direction for future research.


\subsection{Cost-aware attacker}
This is already the strongest whitebox attack. we think the difference is that
the attacker can optimize for minimizing the cost, instead of $L_1$ sum.
In our future work.
We are the first to give an estimation of economic evasion cost in this research area.




==> features.tex <==
\section{Security Applications and Features}

\subsection{Choose Security Applications}

Ransom emails (we need more features than text).

Twitter spam.

\subsection{Categories of Features}

Look at their discussion section and see what they argue.

Features can be categorized into Boolean, Numeric and Categorical ones.
Researchers have argued that if single feature values of Boolean and Numeric types keep increasing or decreasing, the attacker's website/tweet/email becomes more suspicious, if nothing else changes.

\textbf{Monotonically Increasing:} e.g., attackers want to use longer redirection chain and more fast-flux IP addresses, to get agility. Can we verify that the models maintain the same malicious prediction if some feature keeps increasing?

\textbf{Monotonically Decreasing:} e.g., (1) attackers prefer to use something new. e.g., newly registered domains, new accounts. (2) spammers reuse hosting infrastructure. Can we verify that the models maintain the same malicious prediction if some feature keeps decreasing? 

\textbf{Something about categorical features:} n-gram? Jaccard distance? Distributional statistics? mean, variance? If it is reduced to mean and variance, can I use the same monotonicity? How relative is it w.r.t. the entire training dataset (some ratio)? Make a box?



==> phishing.tex <==
%\section{Spearphishing Detection}
%
%This section applies our training method to the spearphishing detection applications.
%
%Three datasets.
%
%Different feature bounds.
%
%Evaluate the cost increase before and after robust training.
%
%Explain how the trees change the features in the predicates after robust training.
%
%Explain the feature importance ranking change.


==> revision.tex <==
\section{Revision Letter}


We greatly appreciate the insightful comments from the reviewers. We have redone the evaluation for the paper, with major changes summarized below.


\begin{enumerate}
%1. Revise the experimental evaluation to include standard evaluation metrics for classifiers, reporting the majority class of the different datasets. Also, discuss hyper-parameter tuning (see reviews for full details).

\item \textbf{Evaluation details.} In Section 4, we have evaluated the classifiers with different standard evaluation metrics including ROC curve and AUC (Figure~\ref{fig:gbdt-aoc}, Figure~\ref{fig:sk-rf-aoc}, Table~\ref{tab:costmodels}).
As stated in Section~\ref{sec:Training Algorithm Evaluation}, in order to reproduce existing results
in related work~\cite{chen2019robust}, we use $0.5$ prediction confidence as the cutoff
to compute the accuracy scores for all trained models.
We have reported the majority class of the four benchmark datasets in Table~\ref{tab:count}.
We have implemented Chen's training algorithm~\cite{chen2019robust} in scikit-learn
to compare against their random forest models in Section~\ref{tab:sklearnrf}.
In Figure~\ref{fig:acc_linf_multiplot} and Figure~\ref{fig:acc_linf_sklearnrf_multiplot},
we have reported the accuracy under attack for
random forest and gradient boosted decision tree models.

\item \textbf{Hyperparameter tuning.} For evaluation using the benchmark datasets,
we have performed grid search for the number of trees and maximum depth
hyperparameters to train a total of 120 random forest models, and we selected the hyperparameters
that generated the best validation accuracy for Table~\ref{tab:sklearnrf} in Section~\ref{subsec:rf}.
For gradient boosted decision trees (GBDT) evaluation, in order to reproduce existing results,
we report results using the same hyperparameters
from~\cite{chen2019robust} in Section~\ref{subsec:gbdt}. However, we have performed
additional hyperparameter grid search by training a total of 140 GBDT models in
Appendix~\ref{appendix:params_gbdt}. We found out that the hyperparameters used in~\cite{chen2019robust}
produced models with accuracy similar to the best ones chosen by the grid search.

% robust accuracy under attacker bounded with $L_1$, $L_2$, and adaptive attackers. 

%2. Discuss the relationship of the proposed technique with traditional attacker models based on mathematical distances.
\item \textbf{Relationship with traditional $L_1$ and $L_2$ attacker models.}
Our current implementation does not support training $L_1$ and $L_2$ attacker models directly,
though we could extend our cost model to support $L_1$-norm bound in training by enforcing
an attack budget, and we could integrate our cost model with~\cite{wang2020ell_p} to support
$L_2$ attack model, which we leave as future work.
However, in Section~\ref{sec:results}, we have demonstrated that using our proposed technique for training,
we can improved the model's robustness against $L_1$ and $L_2$ based attacks as well.
Moreover, compared to Chen's algorithm, we can obtain stronger
robustness against $L_1$ and $L_2$ attacks while achieving better model performance.

%3. Revise the introduction and the abstract to make them clearer, as suggested by the reviewers.
\item \textbf{Revise introduction and abstract.} We have revised introduction and abstract to provide a clearer explanation of our cost model. We motivate the need for modeling feature manipulation cost and cost-aware training approach with a new example in Figure~\ref{fig:motivation}.

%4. Improve the related work section by expanding the comparison with previous work to better assess its strengths and weaknesses. Also, include a discussion on the relationships with the threat model in [A], the tree learning algorithm in [B] and the framework in [C]
\item \textbf{Expanding comparison with previous work.} In Section~\ref{subsec:Related Work}, we have provided detailed comparisons against the threat model and the training algorithm in~\cite{calzavara2019adversarial,calzavara2020treant}.
We have also discussed the relationship of our cost factors with the framework in~\cite{pierazzi2020intriguing}.

%5. Discuss accuracy vs. robustness tradeoffs, including varying the size of the bounding box. How much does this affect the accuracy and robustness of the model?

\item \textbf{Tradeoffs between accuracy and robustness.} In Section~\ref{subsubsect:Box Constraint Specification}
and Section~\ref{sec:results}, we have specified and trained 19 different cost models under different sizes of bounding box and cost-driven constraints, belong to four different cost families. Among them, three cost families (14 models) use
tree categories of feature manipulation cost instead of four.
We compared the model performance and robustness against regular training and
traditional $L_\infty$ based cost models on Twitter Spam dataset in Table~\ref{tab:costmodels}.
Furthermore, in Section~\ref{sec:discussion}, we have discussed the tradeoffs between robustness and accuracy.

%[A] Calzavara Stefano, Claudio Lucchese, and Gabriele Tolomei. "Adversarial Training of Gradient-Boosted Decision Trees." CIKM 2019.

%[B] Calzavara et al. "Treant: Training Evasion-Aware Decision Trees" (https://arxiv.org/abs/1907.01197)

%[C] Pierazzi et al. "Intriguing Properties of Adversarial ML Attacks in the Problem Space". S&P 2020.

\item \textbf{Scalability and generalization.} We have discussed scalability and generalization of our proposed technique
in Section~\ref{sec:discussion}.

\item \textbf{Others.} We have explained the reasons for small number of trees for the breast cancer GBDT model 
in Section~\ref{subsec:gbdt},
and the anomalous low false positive rate for ijcnn1 random forest model in Section~\ref{subsec:rf}. We will release our implementation to the community.

\end{enumerate}

